Historical Gradient Reconstruction for Adaptive Federated Continual Learning

Federated continual learning (FCL) must balance the acquisition of new knowledge with the retention of earlier knowledge distributed across heterogeneous clients. Gradient-based task weighting offers a way to adapt this balance, but choosing the weights requires historical gradients from data distributed across clients. Private replay buffers provide only a local view of past data, while shared historical gradients can become inaccurate as clients update their models. We propose FedGRIT (Federated Gradient Reconstruction for Incremental Training), a replay-based framework that reconstructs historical gradients to guide adaptive local updates. By aggregating task-specific gradients and compact curvature information, FedGRIT enables clients to reconstruct historical gradients at their own changing models and adapt task weights without cross-client communication at every step. Periodic refreshes and two-stage curvature compression support repeated sharing. We derive conditional historical-loss retention and weighted stationarity bounds under partial participation, separating the effects of stochasticity, local training, and client heterogeneity. Across four class- and domain-incremental benchmarks, FedGRIT achieves the highest mean final accuracy among the evaluated methods with ablations examining shared reconstruction and adaptive weighting.

==> section/Sec2-Related_Work.tex <==
\section{Related Work}
\subsection{Continual Learning}
Continual Learning aims to enable a model to sequentially learn knowledge from evolving tasks while mitigating catastrophic forgetting of previously learned knowledge. Existing approaches can be categorized into replay-based, regularization-based, and architecture-based methods. Replay-based methods maintain a limited memory of selected previous samples and jointly incorporate them with the current data during training~\citep{chaudhry2019tinyepisodicmemoriescontinual, Rebuffi2017iCaRL, wu2018memory}. Regularization-based methods preserve previous predictions through knowledge distillation and prevent the model from deviating from the previous optimal model~\citep{Kirkpatrick2017EWC, LiHoiem2017LwF, ritter2018online, li2025became}. Architecture-based methods mitigate catastrophic forgetting by expanding the network or task-specific parameters to isolate the information learned from different tasks~\citep{mallya2018packnet, Liang2023Adaptive}. 

\subsection{Federated Continual Learning}
Federated Continual Learning can be regarded as an expansion of conventional continual learning in the federated setting, which enables clients to sequentially train the model cooperatively, so the main types of FCL can also be categorized into these three types~\citep{yoon2021federated, usmanova2022federated, babakniya2023data, wuerkaixi2025accurate}. However, a key distinction between the two settings lies in information communication, as the communication between clients and the server in FCL needs to account for limited bandwidth and communication costs~\citep{wu2021fast, zhang2023communication, li2024towards, paul2023masked}. In addition, FCL introduces task-level asynchrony besides the communication asynchrony inherited from conventional FL, where different clients may simultaneously train on different tasks due to the heterogeneous task sequences of different clients. FedSpace addresses this asynchrony through prototype aggregation, representation alignment and a modified aggregation policy, enabling knowledge sharing among different clients~\citep{shenaj2023AFCL}, and C$^2$-AFCL introduces a two-stage orthogonal calibration mechanism to mitigate both client and task drift caused by asynchronous client updates~\citep{li2026crosstask}.
{
HERO~\citep{nguyen2026hero} distinguishes client data skew from client task-order mismatch, enabling these dimensions of FCL heterogeneity to be evaluated separately. \Adaptive focuses on the former under a shared task sequence: clients contribute different replay-gradient and curvature estimates for the same historical task, which are aggregated to support adaptive local training. Extending this protocol to client-specific task orders requires accounting for differences in task availability and current versus historical status across clients.}




\subsection{Hessian-informed Continual Learning}
Second-order information has been widely explored in CL to preserve previously acquired knowledge. For all Hessian-based methods, the problem which can not be overlooked is how to find the Hessian matrix. Since forming the full Hessian causes unnecessary computation and storage costs, recent studies focus on using more efficient approximation approaches to recover the Hessian information while training.  The Fisher information matrix is one of the most widely used approximation methods, whose diagonal entries are commonly employed to measure the importance of parameters, but it only captures parameter-wise information while ignoring the correlations among parameters, leading to substantial approximation errors~\citep{Kirkpatrick2017EWC, shoham2019overcomingforgettingfederatedlearning, liu2022continual}. As an alternative to the Fisher information matrix, ~\citet{daxberger2023improving} use the generalized Gauss–Newton (GGN) matrix to provide a more accurate curvature approximation for previous-gradient reconstruction. Another challenge of utilizing Hessian information in CL setting is to prevent the model parameters from deviating significantly from the point at which the Hessian was computed. ~\citet{wu2024meta} and ~\citet{li2026converge} employ iterative strategies to update the Hessian to improve the accuracy of approximation by maintaining up-to-date curvature information while approximating. However, effectively maintaining and updating Hessian information in distributed learning settings remains largely underexplored.


